Orthogonalized ALS: A Theoretically Principled Tensor Decomposition Algorithm for Practical Use

The popular Alternating Least Squares (ALS) algorithm for tensor decomposition is efficient and easy to implement, but often converges to poor local optima---particularly when the weights of the factors are non-uniform. We propose a modification of the ALS approach that is as efficient as standard ALS, but provably recovers the true factors with random initialization under standard incoherence assumptions on the factors of the tensor. We demonstrate the significant practical superiority of our approach over traditional ALS for a variety of tasks on synthetic data---including tensor factorization on exact, noisy and over-complete tensors, as well as tensor completion---and for computing word embeddings from a third-order word tri-occurrence tensor.

==> discussion.tex <==

\section{Discussion}
We have restricted our attention to symmetric tensors in this work, but we believe our techniques can also be used to analyze asymmetric tensor power method updates. We have also not analyzed the stability of our analysis to perturbations, and leave that as a point of future work.

Our work also suggests several bold directions for applications of tensor methods. The orthogonalization step is usually just a few lines of code, and can easily be added to existing highly-optimized tensor decomposition toolboxes. It would be interesting to see if it can improve performance on current applications of tensors. Intuitively, we expect the most gains where the factors are close to incoherent and have large difference in weights. We are also exploring variants such as partially orthogonalizing the factor matrix at each step and stopping orthogonalization after a few initial iterations.

==> g_notes.tex <==
in intro add bit about how many practical machine learning researchers espouse the view that tensor methods are useless. 

this should be heyday of tensors, with rise of multi-modal measurements, language, IoT, etc.

instead of focussing on issues with current stuff, maybe start with desiderata.






build->builds on

nth directiuon OBTAINED by stacking

The difficulty...

hence it is useful to understand.


add comment, we believe the algorithm results and proof approach extend easily to the higher order tensor..

Section 4:  not just 

King -> king


==> intro.tex <==

\section{Introduction}

Tensor methods have become extremely useful tools for guaranteed learning of machine learning models and have been successfully applied to obtain guarantees for topic modeling, community detection \cite{anandkumar2014atensor} and learning graphical models with guarantees via the method of moments\cite{anandkumar2014btensor}. The key property of tensors which makes them extremely useful in theory is that they have a unique decomposition under mild conditions on the factor matrices, for example tensors have a unique decomposition whenever the factor matrices are full rank. However, tensor methods have not been as successful in practical applications as suggested by their success in theory. There could be multiple reasons for this. It is possible that tensor methods are inherently not useful in practice as the regime under which we can successfully recover tensors (tensor decomposition is NP-Hard in the worst-case \cite{hillar2013most} \cite{haastad1990tensor}) is not interesting, or is already covered by simpler methods like matrix factorizations. It is also possible that tensor methods have large sample complexities due to the extra dimensions which have to be filled, and the number of samples required is too high for current datasets. 

In this paper, we take a different view that the reason for tensor methods not achieving breakthrough success in practice is that our algorithmic toolbox for tensors is sill limited and the known algorithms suffer from drawbacks in theory and practice. Ideally, we would like to have tensor decomposition algorithms which extend easily to large tensors (which would possibly be very sparse) and offer guarantees under some plausible conditions. Currently the most popular algorithm for tensor decomposition is alternating least squares (ALS) and it has been described as the ``workhorse'' for tensor decomposition \cite{kolda2009tensor}. The method involves fixing the factors along two modes of the tensor and performing least squares update on the third mode. It is easy to implement with numerous publicly available optimized packages. It is also easily parallelizable and can handle very large tensors if they are sparse \cite{smith2015dms}. However, ALS is known to suffer from local optima and slow convergence, and good conceptual understanding is still lacking. Though we cannot hope for guaranteed tensor decomposition in all cases, we show that ALS suffers from drawbacks even in simple cases which could arise in practice. More sophisticated methods have been proposed via simultaneous diagonalization and higher-order SVD \cite{de2006link}, and initialization schemes for ALS which use these techniques are also known. However, this requires solving a linear system of size $O(d^4)$, where $d$ is the dimension of the tensor, and is hence too expensive for large tensors. 

Another popular algorithm for tensor decomposition is the tensor power method, which is the tensor analog of the matrix power method for computing eigenvectors. The tensor power method is equivalent to performing successive rank-1 ALS decompositions. Recent work by Anandkumar et al. \cite{anandkumar2014guaranteed} established guarantees for the tensor power method. The authors show that tensor power method updates converge locally for random tensors with $k<o(d^{1.5})$ and used SVD based initialization to get global convergence for $k=O(d)$. However, the authors point out that SVD based initialization is again expensive and hence it's desirable to initialize randomly. But we show that random initializations suffers from the drawback that a prohibitively large number of initializations are required to recover smaller factors.

In this work we propose Orthogonalized ALS (Orth-ALS), a simple modification to ALS which ensures guaranteed recovery of all the factors with random initialization under natural constraints on the incoherence between the factors. Our analysis technique for proving convergence of Orth-ALS also lets us improve the guarantees for the tensor power method. We show the following improvement over current results-
\begin{enumerate}
	\item Tensor power method with random initialization converges to one of the factors with small residual error from \emph{random} initialization for $k=o(d)$ for random tensors. 
	\item We show conditions for local and global convergence with random initialization for worst-case tensors, characterized only by the incoherence property of the tensor.
	\item We show that both the global and local rate of convergence is \emph{quadratic} and hence the method converges extremely fast in $O(\log \log k)$ steps.
	\item We also show that orthogonalizing the initial random estimates with respect to previously extracted factors lets us recover all $k$ factors via $k$ random initializations.
\end{enumerate}

We demonstrate the improvements achieved by Orth-ALS via experiments on random tensors. We also apply our algorithm to the task of learning word embeddings, and show that orthogonalization improves the quality of the embeddings.

The rest of the paper is organized as follows- Section 2 introduces the required notation. In Section 3 we discuss the ALS algorithm and the tensor power method. In Section 4 we introduce Orth-ALS. We state our convergence results in Sections 5 and 6. The experimental results are in Section 7. The proof details have been deferred to the appendix.

==> intro_copy.tex <==

\section{Introduction}

From a theoretical perspective, tensor methods have become an incredibly useful and versatile tool for learning a wide array of popular models, including topic modeling \cite{anandkumar2012spectral}, mixtures of Gaussians \cite{ge2015learning}, community detection \cite{anandkumar2014atensor}, and learning graphical models with guarantees via the method of moments \cite{anandkumar2014btensor} \cite{chaganty2014estimating}. The key property of tensors that enables these provable guarantees is that tensors have a unique decomposition under mild conditions on the factor matrices \cite{kruskal1976more} \cite{kruskal1977three}, for example tensors have a unique decomposition whenever the factor matrices are full rank. As tensor methods naturally model three-way (or higher-order) relationships, it would seem reasonable to think that tensor methods should be enjoying a practical heyday, due to rise of multi-modal measurements (e.g. measurements taken by Internet of Things devices, etc) and the numerous practical applications involving high order dependencies, such as natural language and genomic settings.   

Sadly, as of yet, tensor methods have not been as successful in practical applications as suggested by their success in theory, and many applied machine learning researchers espouse the view that tensor methods are simply not useful in practice.  There are several possible explanations for the practical limitations of these methods.  Perhaps the regime under which we tensor methods can successfully recover accurate decompositions is not interesting, or is already solvable by simpler methods like matrix factorizations (tensor decomposition is NP-Hard in the worst-case \cite{hillar2013most} \cite{haastad1990tensor}).  Or maybe the additional sample complexity of tensor methods is too high due to the extra dimensions which have to be estimated, and the number of samples required to reap the benefits of additional dimensions exceeds present current datasets and computational capabilities.

There is a further possibility.  Perhaps the explanation for why tensor methods have not (yet) achieved greater practical use is that the tensor decomposition algorithms hitherto proposed and employed either have strong provable success guarantees but are computationally expensive (though still polynomial time)---either requiring an expensive initialization phase, or being unable to leverage the sparsity of the input tensor, or are efficient to implement but fail to compute an accurate decomposition in many natural settings---the Alternating Least Squares (ALS) algorithm falls in this category and is, by far, the most widely employed decomposition algorithm despite its often poor performance and propensity for getting stuck in local optima (which we demonstrate).   

In this paper we propose an alternative decomposition algorithm, ``Orthogonalized Alternating Lease Squares'' (Orth-ALS) that is both extremely simple and efficient, as well as having strong provable recovery guarantees.  This algorithm is a simple modification of the ALS algorithm to periodically ``orthogonalize'' the estimates of the factors.  From the practical side, this algorithm enjoys all the benefits of the standard ALS algorithm, namely simplicity and computational efficiency/scalability.  Additionally,  the quality of the recovered factors is \emph{substantially} better than the factors recovered by standard ALS.   As we show, on synthetic low-rank tensors, this algorithm consistently recovers the true factors, while standard ALS often falters in local optima and fails both in recovering the true factors and in recovering an accurate low-rank approximation to the original tensor.  We also applied Orth-ALS to a  large 3-tensor of word co-occurrences to compute ``word embeddings''.\footnote{Word embeddings are vector representations of words, which can then be used as features for higher-level machine learning.  Word embeddings have rapidly become the backbone of many downstream natural language processing tasks (see, e.g.~\cite{mikolov2013distributed}).}  The embedding produced by our Orth-ALS algorithm is \emph{significantly} better than that produced by standard ALS, as we quantify via the performance of the resulting word embeddings on three standard NLP datasets that test the ability of the embeddings to answer basic analogy tasks (i.e. ``puppy is to dog'' as ``??? is to cat'') and semantic word-similarity tasks.   Together, these results support our optimism that, with better algorithms, tensor methods may achieve the practical success that the theory portends.  

Beyond the practical benefits of Orth-ALS, we also consider its theoretical properties.  We show that Orth-ALS provably recovers all factors under \emph{random} initialization for worst-case tensors as long as the tensor satisfies an \emph{incoherence} property (which translates to the factors of the tensors having small correlation with each other), which is satisfied by random tensors with rank $k=o(d^{0.25})$ where $d$ is the dimension of the tensor.   This requirement that $k=o(d^{0.25})$ is significantly worse than the best known provable recovery guarantees for polynomial-time algorithms on such tensors---the recent work~\cite{ma2016polynomial} succeeds even in the over-complete setting with $k=o(d^{1.5})$.  Nevertheless, our experiments support our belief that this shortcoming is more a property of our analysis than the algorithm itself.  Additionally, for many practical settings, particularly natural language tasks, the rank of the recovered tensor is typically significantly sublinear in the dimensionality of the space, and the benefits of an extremely efficient and simple algorithm might outweigh limitations on the required rank for provable recovery.

Finally, as a consequence of our analysis technique for proving convergence of Orth-ALS, we also improve the known guarantees for the tensor power method. We show that the tensor power method with \emph{random} initialization converges to one of the factors with small residual error for rank $k=o(d)$, where $d$ is the dimension. We also show that the convergence rate is \emph{quadratic} in the dimension. \citet{anandkumar2014guaranteed} had previously shown local convergence of the tensor power method with a linear convergence rate (and also showed global convergence via a SVD-based initialization scheme, obtaining guaranteed tensor decomposition for the first time for non-orthogonal tensors).  Our new results, particularly this faster convergence rate, provide some deeper insights into the behavior of this popular algorithm.


\iffalse


should be modest, note that $d^{1/4}$ is much worse rank requirement than best poly-time algorithms.  [though optimistic we are optimistic that this is a property of the analysis rather than the algorithm, as our experiments suggest.]  




e demonstrate the improvements achieved by Orth-ALS via experiments on random tensors. In the spirit of trying to make tensor methods feasible on big data applications, we also apply tensor decomposition to the task of learning word embeddings. Word embeddings are vector representations of words which have become the backbone of many downstream natural language processing tasks \cite{mikolov2013distributed}.  Because tensors have the ability to capture three-way relationships among words, we believe tensor methods should help in improving the quality of word embeddings. Learning word embeddings using tensors also presents a challenge for many tensor decomposition algorithms, because decomposing the tensor efficiently necessitates efficient runtime, good parallel performance and handling of sparse tensors. We  apply our algorithm to the task of learning word embeddings, and show that orthogonalization using the Orth-ALS algorithm improves the quality of the embeddings.


breakthrough success in practice is that our algorithmic toolbox for tensors is sill limited and the known algorithms suffer from significant drawbacks in theory and practice. Ideally, we would aspire for a tensor decomposition algorithm which has at least the following desiderata. The algorithm should extend easily to large tensors (which could possibly be very sparse) and be easily parallelizable in order to scale to large datasets. Preferably, the algorithm should be easy to implement and conceptually simple. The algorithm should also ideally have some convergence guarantees and not suffer from local optima under realistic conditions on the tensor. Algorithms which work with random initialization are also much better suited to applications versus algorithms requiring sophisticated initialization schemes.


As a step towards realizing these goals,  we propose Orthogonalized ALS (Orth-ALS), a simple modification to the vastly popular Alternating Least Squares(ALS) algorithm. Being a simple modification of the ALS algorithm, it inherits many of the nice properties of ALS: simplicity, numerous optimized packages and easily parallelizable and scalable to large and sparse databases. In contrast to ALS though (which has  known convergence issues and suffers from local optima even under realistic scenarios), 

W
\fi


The rest of the paper is organized as follows- Section \ref{sec:notation} introduces the required notation. In Section \ref{sec:back} we discuss related work.  Section \ref{sec:orthals} introduces and motivates Orth-ALS, and states the convergence guarantees. We state our convergence results for the tensor power method in Section \ref{sec:tpm}. The experimental results, on both synthetic data and the NLP tasks are discussed in Section \ref{sec:exp}. Proof details have been deferred to the Appendix.

==> local.tex <==
\section{Local convergence}

\localconvergence*
\begin{proof}
	
	Without loss of generality, let the first factor $A_1$ have the largest correlation with the initial estimate. As before, we normalize all the correlations by the correlation of the largest factor, let $\hat{a}_{i,t+1} = \frac{a_{i,t}}{a_{1,t}}$ and normalize all the weights by the weight of the largest factor, $\hat{w}_{i} = \frac{w_{i}}{w_{1}}$. The update equations in terms of the ratio of correlations $\hat{a}_{i,t}$ are-
	\begin{align}
	\hat{a}_{i,t+1} &=\frac { \hat{w}_i \hat{a}_{i,t}^2+ c_{i,1}+ \sum_{j: j \ne \{i,1\}}^{}c_{i,j}\hat{w}_j \hat{a}_{j,t}^2}{1+\sum_{j: j \ne 1}^{}c_{1,j}\hat{w}_j \hat{a}_{j,t}^2}
	\end{align}
	By Lemma \ref{local_induction}, $\hat{w}_j\hat{a}_{j,t}^2 \le \gamma/(k c_{\max})^2, \forall j \ne 1$ hence $\sum_{j}^{}|c_{i,j}\hat{w}_j \hat{a}_{j,t}^2| \le \gamma/(kc_{\max}) < 1; \forall \; i$. 
	\begin{align}
	\frac{1}{1+\sum_{j: j \ne 1}^{}c_{1,j}\hat{w}_j \hat{a}_{j,t}^2} = 1 - \sum_{j: j \ne 1}^{}c_{1,j}\hat{w}_j \hat{a}_{j,t}^2+\epsilon_1
	\end{align}
	where $|\epsilon_1| \le \Big|\sum_{j: j \ne 1}^{}c_{1,j}\hat{w}_j \hat{a}_{j,t}^2\Big|^2$.
	We can now rewrite the updates for $\hat{a}_{i,t+1}$ as-
	\begin{align}
	\hat{a}_{i,t+1} &= \Big(c_{i,1}+\hat{w}_i \hat{a}_{i,t}^2 +\sum_{j: j \ne \{i,1\}}^{}c_{i,j}\hat{w}_j \hat{a}_{j,t} ^2\Big)\Big(1-\sum_{j: j \ne 1}^{}c_{1,j}\hat{w}_j \hat{a}_{j,t}^2+\epsilon_1\Big)
	\end{align}
	Let $\rho_{i,t}=c_{i,1}+\hat{w}_i \hat{a}_{i,t}^2 +\sum_{j: j \ne \{i,1\}}^{}c_{i,j}\hat{w}_j \hat{a}_{j,t} ^2 $. By Lemma \ref{local_induction}, $|\rho_{i,t}| \le \gamma$. Therefore-
	\begin{align}
	\hat{a}_{i,t+1} &= c_{i,1} + \hat{w}_i \hat{a}_{i,t}^2 +\sum_{j: j \ne \{i,1\}}^{}c_{i,j}\hat{w}_j \hat{a}_{j,t}^2 -\rho_{i,t}\sum_{j: j \ne 1}^{}c_{1,j}\hat{w}_j \hat{a}_{j,t}^2+\rho_{i,t}\epsilon_1\\
	\implies \Big|\hat{a}_{i,t+1}\Big| &\le \Big| c_{i,1} \Big| + \Big|\hat{w}_i\hat{a}_{i,t}^2\Big| +\Big|\sum_{j: j \ne \{i,1\}}^{}c_{i,j}\hat{w}_j \hat{a}_{j,t}^2 \Big|+\Big|\rho_{i,t}\sum_{j: j \ne 1}^{}c_{1,j}\hat{w}_j \hat{a}_{j,t}^2\Big| +\Big|\rho_{i,t}\epsilon_1\Big|\\
	\implies \Big|\hat{a}_{i,t+1}\Big| &\le \Big|c_{i,1} \Big| + \Big|\hat{w}_i\hat{a}_{i,t}^2\Big| +\Big|\sum_{j: j \ne \{i,1\}}^{}c_{i,j}\hat{w}_j \hat{a}_{j,t}^2 \Big|+\gamma\Big|\sum_{j: j \ne 1}^{}c_{1,j}\hat{w}_j \hat{a}_{j,t}^2\Big| +\gamma\Big|\epsilon_1\Big|\label{iter_local}
	\end{align}
	Now consider the recursion-
	\begin{align}
	\beta_{0} &= \max_{i\ne 1}{\Big|{w_i} \hat{a}_{i,0}\Big|} \label{beta_1_local}\\
	\beta_{t+1} &= \gamma c_{\max} + \beta_{t}^2 + 3\gamma^2 k \beta_{t}^2c_{\max}\label{beta_2_local}
	\end{align}
	By Lemma \ref{local_induction}, $|{w_i}\hat{a}_{i,t}|\le \beta_t, \;\forall\; i \ne 1$. Hence as before, we will analyze the iterations of $\beta$ instead of keeping track of the different $a_{i,t}$.
	\begin{lemma}\label{local_induction}
		The iterates at time $t$ satisfy the following-
		\begin{enumerate}
			\item  $|\hat{w}_j\hat{a}_{j,t}| \le \beta_t\;\forall \;t$
			\item $|\rho_{i,t}| \le \gamma\;\forall \;t$
			\item $|\hat{a}_{j,t}-c_{i,1}|\le 2\beta_{t-1}^2$
		\end{enumerate}
	\end{lemma}
	\begin{proof}
		We will prove the results by induction. By definition $|\hat{w}_j\hat{a}_{j,0}| \le \beta_0$, hence the base case is correct. Let the statement be true after $m$ steps. Note that by Lemma \ref{iteration_local}, $\beta_m \le O(1/(k c_{\max})) \implies |\hat{w}_j\hat{a}_{j,t}| \le O(1/(k c_{\max}))  \implies \hat{w}_j\hat{a}_{j,t}^2 \le O(1/(k c_{\max})^2)$.[add lemma] Also,
		\begin{align}
		\rho_{i,m}&= c_{i,1}+\hat{w}_i \hat{a}_{i,m}^2 +\sum_{j: j \ne \{i,1\}}^{}c_{i,j}\hat{w}_j \hat{a}_{j,m} ^2\\
		\implies \Big|\hat{w}_i\rho_{i,m}\Big| &\le \Big|\hat{w}_ic_{i,1}\Big|+\Big|\hat{w}_i^2 \hat{a}_{i,m}^2\Big| + \Big|\sum_{j: j \ne \{i,1\}}^{}c_{i,j}\hat{w}_j \hat{w}_i\hat{a}_{j,m} ^2\Big|\\
		&\le \gamma c_{\max} + \beta_m^2 + \gamma k c_{\max} \beta_{m}^2\\
		&\le \beta_{m+1}^2 \le 1
		\end{align}
		Hence $|\rho_{i,m}|\le \gamma$. Therefore, by Eq. \ref{iter_local},
		\begin{align}
		\Big|\hat{w}_i\hat{a}_{i,t+1}\Big| &\le \Big|\hat{w}_ic_{i,1} \Big| + \Big|\hat{w}_i^2\hat{a}_{i,t}^2\Big| +\Big|\sum_{j: j \ne \{i,1\}}^{}c_{i,j}\hat{w}_i\hat{w}_j \hat{a}_{j,t}^2 \Big|+\gamma\Big|\sum_{j: j \ne 1}^{}c_{1,j}\hat{w}_i\hat{w}_j \hat{a}_{j,t}^2\Big| +\gamma\Big|\hat{w}_i\epsilon_1\Big|\\
		&\le \gamma c_{\max} + \beta_m^2 + 3\gamma^2 k c_{\max} \beta_{m}^2\\
		&\le \beta_{m+1}
		\end{align}
		To show that $|\hat{a}_{j,t}-c_{i,1}|\le 2\beta_{t-1}^2$ we use Eq. \ref{recon} and repeat the steps used to show that $|\hat{w}_j\hat{a}_{j,t}| \le \beta_t\;\forall \;t$.
	\end{proof}
	\begin{lemma}\label{iteration_local}
		$\beta_t \le 2\gamma c_{\max} \; \forall \; t\ge O(\log \log k)$, also $\beta_t \le O(1/(k c_{\max})) \; \forall \; t$. 
	\end{lemma}
	\begin{proof}
		We divide the updates into two stages-
		\begin{enumerate}
			\item $\frac{1}{4 k} \le \beta_t^2$:
			
			Note that $k c_{\max} >1$ hence $\beta_t^2 < k  c_{\max}\beta_t^2$. As $\frac{1}{4 k} \le \beta_t^2$, $c_{\max}\le 4k c_{\max} \beta_{t}^2$. Hence we can write:
			\begin{align}
			\beta_{t+1} &\le  \gamma c_{\max} +  4\gamma k c_{\max} \beta_{t}^2\\
			&\le 5\gamma k c_{\max} \beta_{t}^2
			\end{align}
			Hence $\beta_{t+1} < 1/(10\gamma k c_{\max})$ if  $\beta_{t} < 1/(10\gamma k c_{\max})$, so  $\beta_{t} < 1/(10\gamma k c_{\max}) \; \forall \; t$. Also,
			\begin{align}
			\beta_{t+1} &\le  (5\gamma k c_{\max}\beta_0)^{2^t}
			\end{align}
			Note that $(5\gamma kc_{\max}\beta_0)^{2^t}\le \frac{1}{4\gamma k}$ for $t=O(\log\log k)$ and hence we stay in this regime for at most $t=O(\log\log k)$ steps.
			\item Note that in the next step $\beta_t \le 2\gamma c_{\max}$.
		\end{enumerate}
	\end{proof}
	Hence $\beta_t\ \le 2\gamma c_{\max}$ for some $t=O(\log \log k)$. By Lemma \ref{induction_global}, $|\hat{a}_{i,t}-c_{i,1}|\le O(c_{\max}^2), i \ne 1$. Hence $|\hat{a}_{i,t} |\le 2c_{\max}$. By Lemma \ref{error_converge}, the error at convergence satisfies $\normsq{A_1 - \hat{x}_{N}} \le O(kc_{\max}^2)$ and the estimate of the weight $bar{w}_1$ satisfies  $|w_1- \bar{w}_1| \le  O(k_{}c_{\max^2})$.
\end{proof}

==> orth_tpm.tex <==

\section{Orthogonal tensor power method}

\begin{algorithm}\caption{Orthogonalized tensor power method}\label{tpm_orth}
	\textbf{Input:} Tensor $T\in \Real^{d\times d\times d}$, number of iterations $N$.
	\begin{algorithmic}[1]
		\For {$i=1:k$}
		\State Initialize $\hat{A}_i, \hat{B}_i, \hat{C}_i \in \Real^d$ uniformly from the unit sphere
		\State Project $\hat{A}_i$ orthogonal to $\{\hat{A}_j, j \in [i-1]\}$ and normalize to have unit norm.
		\State Project $\hat{B}_i$ orthogonal to $\{\hat{B}_j, j \in [i-1]\}$ and normalize to have unit norm.
		\State Project $\hat{C}_i$ orthogonal to $\{\hat{C}_j, j \in [i-1]\}$ and normalize to have unit norm.
		\For {$t=1:N$}
		\State Rank-1 ALS/Power method updates-$x_{t+1}^{(\tau)}  = T_{(1)}(\hat{C}_i  \odot \hat{B}_i )$
		\State Rank-1 ALS/Power method updates-$y_{t+1}^{(\tau)}  = T_{(2)}(\hat{C}_i  \odot \hat{A}_i )$
		\State Rank-1 ALS/Power method updates-$z_{t+1}^{(\tau)}  = T_{(3)}(\hat{B}_i  \odot \hat{A}_i )$
		%\begin{align}
		%\hat{x}_{t+1} = \frac{T(I, \hat{x}_t, \hat{x}_t)}{\norm{T(I, \hat{x}_t, \hat{x}_t}}
		%x_{t+1}^{(\tau)}  \leftarrow T_{(1)}(\hat{x}_t^{(\tau)}  \odot \hat{x}_t^{(\tau)} )
		%\end{align}
		\State Set $\hat{A}_i  = x_{t+1}^{(\tau)} /\norm{x_{t+1}}^{(\tau)}$, $\hat{A}_i  = y_{t+1}^{(\tau)} /\norm{y_{t+1}}^{(\tau)} $, $\hat{A}_i = z_{t+1}^{(\tau)} /\norm{z_{t+1}}^{(\tau)} $
		\EndFor
		\State Estimate weights $\hat{w}_i  = T(\hat{A}_i , \hat{B}_i, \hat{C}_i )$
		%\begin{align}
		%\hat{w}^{(\tau)}  = T(\hat{x}_N^{(\tau)} , \hat{x}_N^{(\tau)} , \hat{x}_N^{(\tau)} )
		%\end{align}
		\EndFor
		\State \textbf{return} $\hat{A}, \hat{B}, \hat{C}, \hat{w}$
	\end{algorithmic}
\end{algorithm}



\modifiedtpmproof*
	\begin{proof}
		The proof idea is simple, we show that with high probability the initialization will have small correlation with the recovered factors after orthogonalization, and then use Theorem \ref{global_convergence} to get convergence to a new factor from this random initialization.
		
\orthini*
	\begin{proof}
		%From Eq. \ref{non_orth_corr} the correlation of all the remaining factors differs by at most a constant multiplicative factor. As the initial vector $X_{m,0}$ is a random vector and $\norm{\Delta_j} \le O(kc_{\max})$, the inner product $X_{m,0}^T \Delta_j$ is less than $kc_{\max}^2$ with high probability. Hence, the correlation of factors $j<m$ with $X_{m,0}$ is shrunk by a factor of $kc_{\max}=O(\log^{-2} k)$. Note that the initial correlations are projections of a random vector onto a fixed direction, and are distributed as Gaussian random variables by the Central Limit Theorem as $d$ is large. The expected value of the maximum of $k$ samples from a $N(0,1)$ distribution is at most $\sqrt{2\log k}$ times hence with high probability no factor $i<m$ will have maximum correlation after the orthogonalization step. Lemma \ref{good_start} can now recursively be applied on all remaining factors, to get the initialization condition.
		
		We first show that $\argmax_i |w_i a_{i,0}| \ge m$. From Lemma \ref{orth_effect}, the ratio of the weighted correlation of all factors $i<m$  with the random initialization and the weighted correlation of all factors $i\ge m$ with the random initialization is shrunk by a factor of $O(k^{-(1+\epsilon)})$ after the orthogonalization step. Hence no factor $i<m$ will have maximum weighted correlation after the orthogonalization step.
		
		Lemma \ref{good_start_whp} can now be applied on all remaining factors, to get the initialization condition. Without loss of generality, assume that $\argmax |w_i a_{i,0}| = m$. Consider the set of factors $A_i, {m\le i\le n}$, let this set be $S$. From Lemma \ref{good_start_whp}, with probability at least $\Big(1-\frac{\log^2 k}{k^{1+0.5\epsilon}}\Big)$, $\Big|\frac{{w_i} a_{i,0}}{{w_m} a_{m,0}} \Big| \le {1-1/k^{1+0.5\epsilon}}, \epsilon>0 \; \forall \; i\ne 1$. Applying Lemma \ref{orth_effect} once more, $|\hat{w}_i\bar{a}_{i,t}| \le \beta_t(1+1/k^{1+\epsilon})), \; \forall \; i > m$, therefore combining Lemma \ref{good_start_whp} and Lemma \ref{orth_effect}, with failure probability at most $\Big(1-\frac{\log^2 k}{k^{1+0.4\epsilon}}\Big)$, $\Big|\frac{w_i\bar{a}_{i,0}}{w_m \bar{a}_{m,0}} \Big| \le {1-1/k^{1+\epsilon}} \; \forall \; i\ne m$ after the orthogonalization step.
		
	\end{proof}
	
	We now apply Theorem \ref{global_convergence} to get global convergence to the $m$th factor.
	
\end{proof}

==> reconstruct_error_old.tex <==
\section{Proof of additional Lemmas}

\goodstart*
\begin{proof}
	The distribution of the correlation between high-dimensional random vectors is very close to a Gaussian because of the Central Limit Theorem. Note that the distribution of $w t$ where $w$ is a scalar and $t\sim N(0,1)$ is identical to the distribution of $u\sim N(0,w^2)$. Hence we'll treat the weights on the factors as standard deviations of the Gaussian random variables. Also, we are only interested in the ratio hence we can standardize all the correlations to be standard normal variables. Let the weighted random variables corresponding to the $k$ factors be denoted by $\{u_1, \dotsb, u_k\}$. Note that the maximum of $k$ samples from a standard Gaussian is less than $O(\sqrt{\log k})$ with high probability and as the maximum ratio of the weights $\gamma$ is a constant, hence the maximum of all the random variables $u_i$ is $O(\sqrt{\log k}) $. We use the following tail bound on the standard Gaussian random variable $u$-
	\begin{align}
	\frac{e^{-t^2/2}}{t\sqrt{2\pi}}\Big(1-\frac{1}{t^2}\Big)\le\Pr[u>t]\le \frac{e^{-t^2/2}}{t\sqrt{2\pi}}
	\end{align}
	Let $l$ be chosen such that-
	\begin{align}
	\sum_{i=1}^k \frac{w_i e^{-l^2/(2w_i^2)}}{l\sqrt{2\pi}} = \frac{1}{2}\\
	\frac{2}{5}\le \sum_{i=1}^k \frac{w_i e^{-l^2/(2w_i^2)}}{l\sqrt{2\pi}}\Big(1-\frac{w_i ^2}{l^2}\Big) \le \frac{1}{2}\\
	\end{align}
	This is possible as $\Big(1-\frac{w_i ^2}{l^2}\Big) \ge \frac{4}{5}\; \forall \;i$. Hence $\frac{2}{5}\le\sum_{i}^{}\Pr[u_i>l] \le \frac{1}{2}$. Let $u=\max_i u_i$. As the $u_i$ are independent,
	\begin{align}
	\Pr[u>l] &= 1- \Pi(1-\Pr[u_i>l])\\
	&= \sum_{i}^{}\Pr[u_i>l] - \sum_{i<j}^{}\Pr[u_i>l]\Pr[u_j>l] + \dotsb (-1)^k \Pi\Pr[u_i>l]
	\end{align}
	As $\sum_{i}^{}\Pr[u_i>l] \le \frac{1}{2}, (\sum_{i}^{}\Pr[u_i>l])^m\le \frac{1}{2^m}$ and as $\Pr[u_i>l]$ are non-negative, we can write-
	\begin{align}
	\Pr[u>l] &\ge \frac{2}{5} - \frac{1}{2^2} - \frac{1}{2^4} -\dotsb - \frac{1}{2^k}\\
	&\ge \frac{2}{5} -\frac{1}{3}\\
	&\ge \frac{1}{15}
	\end{align}
	
%		\begin{align}
%		\frac{\sum_{i=1}^{k}\Pr[-l\le u_i\le l]}{k} \le 1-\frac{2\log k}{k}
%		\end{align}
%		Let $u=\max_i u_i$. As the $u_i$ are independent,
%		\begin{align}
%		\Pr[u>l] &= 1- \Pi_i \Pr[|u_i|\le l]
%		\end{align}
%		By the AM-GM inequality-
%		\begin{align}
%		\Pi_i \Pr[|u_i|\le l] &\le \Big(\frac{\sum_{i=1}^{k}\Pr[|u_i|\le l]}{k}\Big)^{k}\\
%		&\le (1-\frac{2\log k}{k})^k\\
%		&\le \frac{1}{k^2}
%		\end{align}
	
	We now upper bound $\Pr[u>l(1-\log^{-1.5} k)]$. We can write,
	\begin{align}
	\Pr[u>l(1-\log^{-1.5} k)] &\le \sum_{i}^{} \Pr[u_i>l(1-\log^{-1.5} k)] \\
	&\le \sum_i \frac{w_i\exp(-\frac{l^2}{2w_i}(1-2/(\log k)^{1.5}+1/(\log k)^{3}))}{\sqrt{2\pi}l(1-\log^{-1.5} k)}\\
	&\le \sum_i \frac{w_i\exp(-\frac{l^2}{2w_i}(1-2/(\log k)^{1.5}))}{0.9\sqrt{2\pi}l}\\
	&\le \sum_i \Big(\frac{\exp({l^2}/({w_i(\log k)^{1.5}}))}{0.9}\Big)\Big(\frac{w_i\exp(-{l^2}/({2w_i}))}{l\sqrt{2\pi}}\Big)
	\end{align} 
	As $l=O(\sqrt{\log k})$ and $w_i$ is constant, $\frac{\exp({l^2}/({w_i(\log k)^{1.5}}))}{0.9}\le 1.1/0.9 \le 1.25$. Hence,
	\begin{align}
	\Pr[u>l(1-\log^{-1.5} k)]  &\le \sum_i 1.25\Big(\frac{w_i\exp(-{l^2}/({2w_i}))}{l\sqrt{2\pi}}\Big)\\
	&\le 0.625
	\end{align}
	Hence with constant probability one of the $u_i$ is larger than $l$ and all others are smaller than $l(1-\log^{-1.5} k)$.
	
\end{proof}

\begin{lemma}\label{error_converge}
	Let $kc_{\max}^2 \le 1/\polylog k$ and $\frac{w_{\max}}{w_{\min}}=\gamma$ (constant). Without loss, of generality assume convergence to the first factor $A_1$. Define $\hat{a}_{i,t} =|\frac{\tilde{a}_{i,t}}{\tilde{a}_{1,t}}|$- the ratio of the correlation of the $i$ and 1st factor with the iterate at time $t$. If $\hat{a}_{i,t} \le  2 c_{\max}$, then $\normsq{A_1 - \hat{x}_{N}} \le O(kc_{\max}^2)$ for all subsequent iterations. Also, the estimate of the weight $bar{w}_1$ satisfies  $|w_1- \bar{w}_1| \le  O(k_{}c_{\max^2})$.
\end{lemma}
\begin{proof}
	Consider any step $\tau$ of the power iterations at the end of which $|a_{i,\tau}|\le 6\gamma c_{\max} \;\forall\; i\ne 1$. Let the first (largest) factor have true correlation $c_1$ with the iterate at time this step and $|w_1 c_1| = \alpha$. Consider the next tensor power method update. From the update formula, the result $\hat{x}_{\tau+1}$ is-
	\begin{align}
	\hat{x}_{\tau+1} = \frac{\sum_{i=1}^{k}w_1\hat{w}_ic_1^2\hat{a}_{i,\tau}^2A_{i}}{\norm{\sum_{i=1}^{k}w_1\hat{w}_ic_1^2\hat{a}_{i,\tau}^2A_{i}}}
	\end{align}
	Let $\kappa = \frac{w_1 c_1^2}{\norm{\sum_{i=1}^{k}w_1\hat{w}_ic_1^2\hat{a}_{i,\tau}^2A_{i}}}$. Hence the estimate at the end of the $m$th iteration is-
	\begin{align}
	\hat{x}_{\tau+1} &= \kappa\sum_{i=1}^{k}\hat{w}_i\hat{a}_{i,\tau}^2A_{i}\\
	&= \kappa(A_1+\sum_{i\ne 1}^{}\hat{w}_i\hat{a}_{i,\tau}^2A_{i})
	\end{align}
	Denote $\sum_{i\ne 1}^{}\hat{w}_i\hat{a}_{i,\tau}^2A_{i} = \hat{\Delta}_1$. Note that  $\norm{\hat{\Delta}_1} \le O({k_{} c_{\max}^2})$ as $|\hat{w}_i\hat{a}_{i,\tau}| \le 2 c_{\max} \implies \hat{w}_i\hat{a}_{i,\tau}^2 \le 4\gamma c_{\max}^2 $ and the factors $A_i$ have unit norm. We can write-
	\begin{align}
	\hat{x}_{\tau+1} &= \kappa(A_1+\hat{\Delta}_1)
	\end{align}
	As $\norm{\hat{x}_{\tau+1}}=1, \kappa = 1/\norm{A_1+\hat{\Delta}_1}$. From the triangle inequality,
	\begin{align}
	& 1-\norm{\hat{\Delta}_1}\le \norm{A_1+\hat{\Delta}_1} \le 1+ \norm{\hat{\Delta}_1}\\
	\implies & 1-O(k_{} c_{\max}^2)\le \norm{A_1+\hat{\Delta}_1} \le 1+ O(k_{} c_{\max}^2)\\
	\implies & \frac{1}{1+O(k_{} c_{\max}^2)} \le \kappa \le  \frac{1}{1-O(k_{} c_{\max}^2)} \\
	\implies & {1-O(k_{} c_{\max}^2)} \le \kappa \le  {1+O(k_{} c_{\max}^2)} 
	\end{align}
	
	We can now write the error  $\norm{A_1-\hat{x}_{\tau+1}} $ as-
	\begin{align}
	\norm{A_1-\hat{x}_{\tau+1}} &=\norm{A_1- \kappa(A_1 + \hat{\Delta}_1)} \\
	&= \norm{A_1(1-\kappa) + \hat{\Delta}_1}\\
	&\le \norm{(A_1(1-\kappa))} + \norm{\hat{\Delta}_1}\\
	&\le |1-\kappa| + O(k_{} c_{\max}^2)\\
	&\le O(k_{} c_{\max}^2)
	\end{align}
	We also show that the error in estimating the weight $w_1$ of factor $A_1$ is small once we have good estimate of the factor.
	\begin{align}
	\bar{w}_1 &= \sum_{i}^{}w_i <\hat{x}_N, A_i>^3\\
	&= \sum_{i}^{}w_i <A_1 + \hat{\Delta}_1, A_i>^3\\
	&= w_1 + O(k_{}c_{\max^2})+\sum_{i\ne 1}^{}w_i <A_1 + \hat{\Delta}_1, A_i>^3\\
	&\le w_1 + O(k_{}c_{\max^2})+ \sum_{i}^{}w_i c_{\max}^3 \label{weight}\\
	&\le w_1 + O(k_{}c_{\max^2})+ w_i kc_{\max}^3\\
	\implies |w_1- \bar{w}_1| &\le  O(k_{}c_{\max^2})
	\end{align}
	where Eq. \ref{weight} follows as $|A_i^T \hat{\Delta}_1 |\le \norm{\hat{\Delta}_1} \le c_{\max}$.
\end{proof}

==> summary.tex <==

\section{Summary of results}

We summarize our results for different settings in this section. Define $c_{\max} = \max_{i,j: i \ne j} |c
_{i,j}$. Intuitively $c_{\max}$ measures the incoherence between the true factors. 

\subsection{Global convergence of tensor power method}
We demonstrate that tensor power method has global convergence with high probability under random initialization in $O(\log\log (k+1/c_{\max}))$ steps under the following assumptions on deterministic tensors-
\begin{enumerate}
	\item \emph{Incoherence}: $c_{\max} \le \frac{1}{k\;\polylog k}$
	\item $\sum_{j}^{}A_j w_j c_{\max}^2 \le O(\frac{\sqrt{k}}{d})$. 
\end{enumerate}

For random tensor we can relax condition 1 to $c_{\max} \le \frac{1}{\sqrt{k}\; \polylog k}$. With high probability this assumption is satisfied for random tensors with $k\le \frac{d}{\polylog k}$. Condition 2 is used to ensure that the error is small when the tensor power method converges. It is similar to incoherence, though we do not prove a formal relation. We show that it is satisfied for random tensors with high probability.

\subsection{Local convergence of tensor power method}
We demonstrate that tensor power method has local convergence in $O(\log\log (k+1/c_{\max}))$ steps under the following assumptions on the tensors and initialization-

\begin{enumerate}
\item \emph{Incoherence}: $c_{\max} \le \frac{1}{\sqrt{k}\;\polylog k}$
\item \emph{Initialization}: The initial estimate $\hat{x}_{0}$ has correlation atleast $\frac{\sqrt{k}}{d}$ with one of the true factors. 
\item $\sum_{j}^{}A_j w_j c_{\max}^2 \le O(\frac{\sqrt{k}}{d})$. 
\end{enumerate}
For random tensor we can relax condition 1 to $c_{\max} \le \frac{1}{{k}^{0.25}\; \polylog k}$.  With high probability this assumption is satisfied for random tensors with $k\le \frac{d^2}{\polylog k}$. The initialization criterion we impose is mild even for highly over complete tensors and as remarked in \cite{anandkumar2014analyzing} such initialization can usually be obtained from data. In  \cite{anandkumar2014sample} the authors use overcomplete tensor decomposition to learn overcomplete latent variable models.

\subsection{Recovering all factors together via Orthogonalized ALS (Algorithm \ref{orth}})

Our global guarantees for the modified version of ALS is the same as our guarantees for the tensor power method iterations-

\begin{enumerate}
	\item \emph{Incoherence, deterministic case}: $c_{\max} \le \frac{1}{k\;\polylog k}$
	\item \emph{Incoherence, random case}: $c_{\max} \le \frac{1}{\sqrt{k}\; \polylog k}$
	\item $\sum_{j}^{}A_j w_j c_{\max}^2 \le O(\frac{\sqrt{k}}{d})$. 
\end{enumerate}


==> tpm.tex <==

%
%\section{Orthogonalized ALS: Convergence guarantees }
%
%In the previous section we analyzed Orthogonalized ALS for the special case of orthogonal tensors. More generally, we can guarantee global convergence of Orthogonalized ALS assuming the factors are sufficiently incoherent-
%
%\begin{restatable}{theorem}{orthalsconvergence}
%	\label{orth_als_convergence}
%	Define $\eta=\max( c_{\max},1/d)$. Let $c_{\max} \le \frac{1}{k \; \polylog k}$ and $\frac{w_{\max}}{w_{\min}}=\gamma$. If the initial estimate for all the factors are initialized randomly from the unit sphere, then the orthogonalized ALS updates converge to the true factors in $O(\log \log k )$ steps per factor, and the error at convergence satisfies $\normsq{A_i - \hat{x}_{N}} \le O(k\eta^2)$ and $|w_1- \bar{w}_1| \le  O(k_{}c_{\max^2})$ for all $i$.
%\end{restatable}
%
%\begin{itemize}
%	\item First consider the case when the rank of the tensor is a constant independent of the dimension. In practice, we only seek a low-rank decomposition of the tensor for many applications. When the rank $k$ is constant, Theorem \ref{orth_als_convergence} provides strong guarantees for worst case tensors. In this case, the factors of the tensor are allowed to have up to $o(1/k^2)$ correlation with each other, which is a constant independent of the dimension $d$. Hence the factors are allowed to have significant correlation with each other in this case, and we can still guarantee global convergence with random initialization for the tensor power method updates.
%	\item For random $d$ dimensional tensors, $c_{\max} = O(1/\sqrt{d})$ which implies that the rank $k$ has to be $o({d}^{0.25})$ to guarantee global convergence with random initialization. 
%\end{itemize}



\section{New Guarantees for the Tensor Power Method}\label{sec:tpm}

As a consequence of our analysis of the orthogonalized ALS algorithm, we also prove new guarantees on the tensor power iteration algorithm. As these may be of independent interest because of the wide use of the tensor power method, we summarize them in this section. We show a quadratic rate of convergence (in $O(\log \log d)$ steps) for random tensors with random initialization.  This contrasts with the analysis of  Anandkumar et al. ~\cite{anandkumar2014guaranteed} who showed a linear rate of convergence ($O(\log d)$ steps) for random tensors, provided an SVD based initialization is employed.% We perform a new analysis of the tensor power method updates and show global convergence of the updates with random initialization.  %Theorem \ref{global_convergence} shows that the tensor power method converges with random initialization as long as the maximum correlation between any two factors is smaller than $\tilde{O}(1/k)$.

\begin{restatable}{theorem}{randomtensor}
	\label{random_tensor}
	Consider a $d$-dimensional rank $k$ tensor $T=\sum_{i=1}^{k}w_i A_i \otimes A_i \otimes A_i$ with the factors $A_i$ sampled uniformly from the $d$-dimensional sphere. Define $\gamma=\frac{w_{\max}}{w_{\min}}$ to be the ratio of the largest and smallest weight. Assume $k  \le d^{1-\epsilon}$ for some $\epsilon>0$. If $x_0\in \Real^d$ is chosen uniformly from the unit sphere, then the tensor power method updates converge to one of the true factors (say $A_1$)  with constant probability over the random initialization in $O(\log \log d )$ steps, and the error at convergence satisfies $\norm{A_1 - \hat{A}_{1}} \le \tilde{O}(1/\sqrt{d})$. Also, the estimate of the weight $\hat{w}_1$ satisfies  $|1- \frac{\hat{w}_1}{w_1}| \le \tilde{O}(1/\sqrt{d})$.
\end{restatable}

\begin{comment}

Our analysis also allows us to obtain a clean characterization for global convergence of the tensor power method updates for worst-case tensors in terms of the incoherence of the factor matrix --

\begin{restatable}{proposition}{globalconvergence}
	\label{global_convergence}
	Consider a $d$-dimensional rank $k$ tensor $T=\sum_{i=1}^{k}w_i A_i \otimes A_i \otimes A_i$. As above, let $c_{\max}=\max_{i \ne j} |A_i^T A_j|$ and  $\gamma=\frac{w_{\max}}{w_{\min}}$ be the ratio of the largest and smallest weight, and assume $\gamma c_{\max} \le \tilde{O}(k^{-2})$. If $x_0\in \Real^d$ is chosen uniformly from the unit sphere, then the alternating least squares updates converge to one of the true factors (say $A_1$)  with constant probability over the random initialization in $O(\log k +\log\log d )$ steps, and the error at convergence satisfies$\normsq{A_1 - \hat{A}_1} \le O(k\max\{c_{\max}^2,1/d^2\})$ and $|1- \frac{\hat{w}_1}{w_1}| \le  O(\max\{c_{\max},1/d\})$.
\end{restatable}

Under milder restrictions on the incoherence of the factor matrix, we also get local convergence of the the tensor power method updates for worst-case tensors given sufficiently high correlation with one of the true factors. More precisely, the initialization conditions in Proposition \ref{local_convergence} are satisfied with an initialization that has correlation at least $O(k/d)$ with one of the true factors and $O(1/\sqrt{d})$ with every other factor. This initialization condition is stronger than the one proposed in \cite{anandkumar2014analyzing} which only needs a correlation of $O(\sqrt{k}/d^{1-\epsilon})$ for some $\epsilon>0$ with one of the true factors. However, our guarantees hold for worst case incoherent tensors in contrast to the guarantees in \cite{anandkumar2014analyzing} which hold for random tensors.
[WHAT IS THE POINT OF THIS?  IS THIS THE KEY LEMMA WE USE TO PROVE THE ABOVE?  IF SO,LETS JUST STATE THIS AND REMOVE ABOVE
\begin{restatable}{proposition}{localconvergence}
	\label{local_convergence}
	Let $\gamma c_{\max} \le \tilde{O}(k^{-0.5})$. If the ratio of the correlations of initial estimate ${X}_{0}$ with some factor (say $A_1$) and any other factor is atleast $O(kc_{\max})$, then the alternating least squares updates converge to $A_1$ in $O(\log \log k )$ steps and the error at convergence satisfies $\normsq{A_1 - \hat{A}_{1}} \le O(kc_{\max}^2)$.
\end{restatable}


The key idea for the analysis for the case when the factors are random is to have a better bound for the term $\sum_{j: j \ne \{i,1\}}^{}c_{i,j}\hat{w}_j \hat{a}_{j,t}^2$ for the random case. In the worst case- the term can be as large as $kc_{\max}\beta_t^2$ if $|\hat{w}_j \hat{a}_{j,t}^2| \le \beta_t^2$. However we show that in the random case we can effectively bound the sum by $\sqrt{k}c_{\max}\beta_t^2$. The fact that the updates converge in a small number of steps ($O(\log \log k)$ steps is crucial to the analysis. In order to bound the $\sum_{j: j \ne \{i,1\}}^{}c_{i,j}\hat{w}_j \hat{a}_{j,t}^2$ term we write down the correlation of the iterate at time $t$ with any factor in terms of the initial correlations with the random initialization. Consider the iterates at time 1 and 2. By the tensor power update equations-
\begin{align}
a_{i,1} &= (w_ia_{i,0}^2 + \sum_{j \ne i}^{}c_{i,j}w_j a_{j,0}^2)\\
a_{i,2} &= (w_ia_{i,1}^2 + \sum_{j \ne i}^{}c_{i,j}w_j a_{j,1}^2)
\end{align}
By expanding $\sum_{j \ne i}^{}c_{i,j}w_j a_{j,1}^2$ in terms of the $a_{i,0}$ terms-
\begin{align}
\sum_{j \ne \{i,1\}}^{}c_{i,j}w_j a_{j,1}^2 &= \sum_{j \ne  \{i,1\}}^{}c_{i,j}w_j \Big(w_ja_{j,0}^2 + \sum_{k \ne j}^{}c_{j,k}w_k a_{k,0}^2\Big)^2\\
&= \sum_{j \ne  \{i,1\}}^{}c_{i,j}w_j \Big(\sum_{k,l}^{}c_{j,k}c_{j,l}w_ka_{k,0}^2w_la_{l,0}^2\Big)\\
&=  \sum_{j \ne  \{i,1\}, k, l}^{}c_{i,j} c_{j,k}c_{j,l}w_jw_kw_la_{l,0}^2a_{k,0}^2
\end{align}

We then use the independence of the $c_{i,j}$ and $a_{i,0}$ terms to prove our bounds. 

We also propose a modification to the tensor power method to have guaranteed recovery of \emph{all} $k$ factors with only $k$ random initializations, in contrast to running the tensor power method sufficiently many times and then clustering all the factors hence obtained. Note that even when all factors have the same weight, the usual tensor power method needs $k\log k$ random initializations to recover all $k$ factors due to the coupon collector phenomena. The orthogonalized tensor power method (Orth-TPM, Algorithm \ref{tpm_orth}) projects the initial random estimate orthogonal to the previously extracted factors, in contrast to orthogonalizing at each step. However, experiments suggest that this milder form of orthogonalization is not as effective as Orth-ALS when the distribution of the weights becomes highly skewed (see Section~\ref{sec:exp}). We show that the modified tensor power method with orthogonal initializations (Orth-TPM, Algorithm \ref{tpm_orth}) recovers all the factors in one-shot under conditions similar to Theorem \ref{orth_als_convergence}.  [WHAT DO YOU MEAN BY ONE SHOT?  rWHERE is ALGORITHM 5?   WHY DO WE HAVE THIS HERE?]

\begin{restatable}{proposition}{modifiedtpmproof}
	\label{modified_tpm_proof}
	Consider a $d$-dimensional rank $k$ tensor $T=\sum_{i=1}^{k}w_i A_i \otimes A_i \otimes A_i$. Define $c_{\max}=\max_{i \ne j} |A_i^T A_j|$ to be the incoherence between the factors and $\gamma=\frac{w_{\max}}{w_{\min}}$ to be the ratio of the largest and smallest weight. Assume $\gamma c_{\max} \le \tilde{O}(k^{-2})$. If the initial estimate for all the factors are initialized randomly from the unit sphere, then the modified tensor power method updates converge to the true factors in $O( k\log k )$ steps, and the error at convergence satisfies (up to relabelling) $\normsq{A_i - \hat{A}_i} \le O(k\max\{c_{\max}^2,1/d^2\})$ and $|1- \frac{\hat{w}_i}{w_i}| \le  O(\max\{c_{\max},1/d\})$ for all $i$.
\end{restatable}

\end{comment}

%Applying Theorem \ref{local_convergenge} for the case of random tensors implies that the tensor power method has local convergence whenever the rank is less than the dimension, up to logarithmic factors. We do not provide a stronger analysis of the updates for the case of random tensors in this case, but believe that our techniques can be extended to show local convergence whenever the rank is less than $o(d^2)$. 
